Open-Vocabulary Federated Learning with Multimodal Prototyping

Existing federated learning (FL) studies usually assume the training label space and test label space are identical. However, in real-world applications, this assumption is too ideal to be true. A new user could come up with queries that involve data from unseen classes, and such open-vocabulary queries would directly defect such FL systems. Therefore, in this work, we explicitly focus on the under-explored open-vocabulary challenge in FL. That is, for a new user, the global server shall understand her/his query that involves arbitrary unknown classes. To address this problem, we leverage the pre-trained vision-language models (VLMs). In particular, we present a novel adaptation framework tailored for VLMs in the context of FL, named as Federated Multimodal Prototyping (Fed-MP). Fed-MP adaptively aggregates the local model weights based on light-weight client residuals, and makes predictions based on a novel multimodal prototyping mechanism. Fed-MP exploits the knowledge learned from the seen classes, and robustifies the adapted VLM to unseen categories. Our empirical evaluation on various datasets validates the effectiveness of Fed-MP.

==> tables/robustness_study.tex <==
\begin{table}[!bht]
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Metrics}    & 30  & 40 & 50   \\ 
\midrule
\multirow{4}{*}{Caltech101}
& $\mathcal{A}$ $\uparrow$      & $0.9936_{\pm 0.0010}$ & $0.9857_{\pm 0.0029}$ & $0.9332_{\pm 0.0197}$ \\
& $\Phi_{P}$    $\uparrow$      & $0.9848_{\pm 0.0030}$ & $0.9700_{\pm 0.0058}$ & $0.8898_{\pm 0.0219}$ \\
& $\Phi_{R}$    $\uparrow$      & $0.9908_{\pm 0.0014}$ & $0.9894_{\pm 0.0020}$ & $0.9784_{\pm 0.0042}$ \\
& $\Phi_{F1}$   $\uparrow$      & $0.9876_{\pm 0.0020}$ & $0.9790_{\pm 0.0038}$ & $0.9238_{\pm 0.0174}$ \\
\midrule
\multirow{4}{*}{UCF101}
& $\mathcal{A}$ $\uparrow$      & $0.9127_{\pm 0.0225}$ & $0.9073_{\pm 0.0352}$ & $0.8818_{\pm 0.0100}$ \\
& $\Phi_{P}$    $\uparrow$      & $0.9212_{\pm 0.0238}$ & $0.9105_{\pm 0.0374}$ & $0.8911_{\pm 0.0126}$ \\
& $\Phi_{R}$    $\uparrow$      & $0.9127_{\pm 0.0255}$ & $0.9073_{\pm 0.0352}$ & $0.8818_{\pm 0.0100}$ \\
& $\Phi_{F1}$   $\uparrow$      & $0.9086_{\pm 0.0298}$ & $0.9013_{\pm 0.0408}$ & $0.8702_{\pm 0.0127}$ \\
% \midrule
% \multirow{4}{*}{FGVC}
% & $\mathcal{A}$ $\uparrow$      & $0.8082_{\pm 0.0199}$ &  &  \\
% & $\Phi_{P}$    $\uparrow$      & $0.8225_{\pm 0.0119}$ &  &  \\
% & $\Phi_{R}$    $\uparrow$      & $0.8014_{\pm 0.0292}$ &  &  \\
% & $\Phi_{F1}$   $\uparrow$      & $0.7842_{\pm 0.0336}$ &  &  \\
\midrule
\multirow{4}{*}{Food101}    
& $\mathcal{A}$ $\uparrow$      & $0.9828_{\pm 0.0005}$ & $0.9827_{\pm 0.0006}$ & $0.9718_{\pm 0.0005}$ \\
& $\Phi_{P}$    $\uparrow$      & $0.9829_{\pm 0.0005}$ & $0.9828_{\pm 0.0006}$ & $0.9731_{\pm 0.0005}$ \\
& $\Phi_{R}$    $\uparrow$      & $0.9828_{\pm 0.0005}$ & $0.9827_{\pm 0.0006}$ & $0.9718_{\pm 0.0005}$ \\
& $\Phi_{F1}$   $\uparrow$      & $0.9828_{\pm 0.0005}$ & $0.9827_{\pm 0.0006}$ & $0.9720_{\pm 0.0005}$ \\ 
\midrule
\multirow{4}{*}{Flower102}  
& $\mathcal{A}$ $\uparrow$      & $0.9098_{\pm 0.0251}$ & $0.9003_{\pm 0.0340}$ & $0.8736_{\pm 0.0240}$    \\
& $\Phi_{P}$    $\uparrow$      & $0.9175_{\pm 0.0224}$ & $0.8886_{\pm 0.0353}$ & $0.8729_{\pm 0.0102}$    \\
& $\Phi_{R}$    $\uparrow$      & $0.9289_{\pm 0.0205}$ & $0.9123_{\pm 0.0319}$ & $0.8945_{\pm 0.0131}$    \\
& $\Phi_{F1}$   $\uparrow$      & $0.9132_{\pm 0.0253}$ & $0.8875_{\pm 0.0391}$ & $0.8684_{\pm 0.0131}$    \\ 
% \midrule
% \multirow{4}{*}{StanfordCars}   
% & $\mathcal{A}$ $\uparrow$    & $0.9721_{\pm 0.0032}$      \\
% & $\Phi_{P}$    $\uparrow$    & $0.9751_{\pm 0.0026}$      \\
% & $\Phi_{R}$    $\uparrow$    & $0.9716_{\pm 0.0033}$      \\
% & $\Phi_{F1}$   $\uparrow$    & $0.9720_{\pm 0.0032}$      \\                                 
\bottomrule
\end{tabular}
}
\caption{Ablation Study.}
\label{tab:ablation}
\end{table}

